Quantum signal processing over SU(N)

Quantum signal processing (QSP) and the quantum singular value transformation (QSVT) are pivotal tools for simplifying the development of quantum algorithms. These techniques leverage polynomial transformations on the eigenvalues or singular values of block-encoded matrices, achieved with the use of just one control qubit. In contexts where the control qubit is used to extract information about the eigenvalues or singular values, the amount of extractable information is limited to one bit per protocol. In this work, we extend the original QSP ansatz by introducing multiple control qubits. We show that, much like in the single-qubit case, nearly any vector of polynomials can be implemented with a multi-qubit QSP ansatz, and the gate complexity scales polynomially with the dimension of such states. Moreover, assuming that powers of the matrix to transform are easily implementable - as in Shor's algorithm - we can achieve polynomial transformations with degrees that scale exponentially with the number of control qubits. This work aims to provide a partial characterization of the polynomials that can be implemented using this approach, with phase estimation schemes and discrete logarithm serving as illustrative examples.

==> contents/apx-single-qubit-proof.tex <==
\section{Proof for single-qubit quantum signal processing}
\label{apx:qsp-single-qubit-proof}

\noindent We present a slightly different formulation of the proof for the already-known single-qubit QSP, which we restate for convenience:

\begin{theoremrestate}{\ref{thm:single-qubit-qsp-analytic}}
    Let $P, Q \in \C[z]$. There exist $A_0, \ldots, A_n \in SU(2)$ such that
    \begin{align*}
        A_n \Tilde{w} A_{n-1} \Tilde{w} \cdots \Tilde{w} A_0 \ket{0} =
        \begin{bmatrix}
            P(z) \\
            Q(z)
        \end{bmatrix}
    \end{align*}
    if and only if
    \begin{enumerate}[(i)]
        \item $\deg P, Q \le n$;
        \item $|P|^2 + |Q|^2 = 1$ for every $z \in U(1)$.
    \end{enumerate}
\end{theoremrestate}
\begin{proof}
    We start with the easy direction: if $n = 0$, then $A_0 \ket{0}$ is a vector containing two complex numbers (i.e., zero-degree polynomials) $p, q$ satisfying $|p|^2 + |q|^2 = 1$. Note that the length-$n$ sequence $(\id, \ldots, \id, A_0)$ produces the same zero-degree polynomial, for any $n$, which will guarantee that any polynomial can be constructed also with longer protocols. For $n > 0$, consider $P', Q'$ of degree $\le n - 1$: we multiply with the $n$-th step
    \begin{align*}
        A_n
        \Tilde{w}
        \begin{bmatrix}
            P' \\ Q'
        \end{bmatrix}
        =: 
        \begin{bmatrix}
            P \\ Q
        \end{bmatrix}.
    \end{align*}
    Condition~(ii) is preserved by unitarity, while the degrees of $P, Q$ are $\le n$ since $P', Q'$ are of degree $\le n - 1$ and $\Tilde{w}$ can only add one degree to the terms of each polynomial.

    The converse also proceeds by induction. For $n = 0$, $P, Q$ are constants, and $A_0 \ket{0}$ can be chosen accordingly. With $n > 0$, we undo the last step:
    \begin{align*}
        (A_n \Tilde{w})^\dag
        \begin{bmatrix}
            P \\ Q
        \end{bmatrix}
        =:
        \begin{bmatrix}
            P' \\ Q'
        \end{bmatrix}.
    \end{align*}
    As before, condition (ii) will be preserved by unitarity, so we only need to choose $A_n$ such that $P', Q'$ will be of degree $\le n - 1$, and the induction hypothesis will imply the claim. For the sake of exposition, let us see what the action of $\Tilde{w}^\dag$ is:
    \begin{align}
        \Tilde{w}^\dag :\ & \begin{bmatrix}
            P(z) \\ Q(z)
        \end{bmatrix}
        \rightarrow
        \begin{bmatrix}
            P(z) \\ z^{-1} Q(z)
        \end{bmatrix} \nonumber \\
        \Tilde{w}^\dag :\ &
        \begin{bmatrix}
            P_0 \\ Q_0
        \end{bmatrix} +
        \begin{bmatrix}
            P_1 \\ Q_1
        \end{bmatrix}
        z + \cdots +
        \begin{bmatrix}
            P_{n-1} \\ Q_{n-1}
        \end{bmatrix}
        z^{n-1} +
        \begin{bmatrix}
            P_n \\ Q_n
        \end{bmatrix}
        z^n \nonumber\\
        \rightarrow &
        \begin{bmatrix}
            0 \\ Q_0
        \end{bmatrix}
        z^{-1} +
        \begin{bmatrix}
            P_0 \\ Q_1
        \end{bmatrix} +
        \begin{bmatrix}
            P_1 \\ Q_2
        \end{bmatrix}
        z + \cdots +
        \begin{bmatrix}
            P_{n-1} \\ Q_n
        \end{bmatrix}
        z^{n-1} +
        \begin{bmatrix}
            P_n \\ 0
        \end{bmatrix}
        z^n.
        \label{eq:one-qubit-poly-shift}
    \end{align}
    \begin{figure}
        \centering
        \input{figures/one-qubit-shift}
        \caption{Visualization of Eq.~(\ref{eq:one-qubit-poly-shift}). The squares represent the coefficients of the two polynomials. Since $\Tilde{w}^{\dag} = \diag(1, z^{-1})$, we are mapping $P(z) \rightarrow P(z), Q(z) \rightarrow z^{-1}Q(z)$, implying that the coefficients of $Q$ are shifted by one degree. The colored squares are the coefficients that end up in front of $z^k$ for $k \not\in [0, n-1]$, so we need to choose $A_n^\dag$ such that these are mapped to $0$ in order to reduce the degree of the polynomial.}
        \label{fig:one-qubit-shift}
    \end{figure}
    \noindent In simple terms, the coefficients of $P$ are left unchanged by $\Tilde{w}$, while the coefficients of $Q$ are shifted by one position to the left (see also Figure~\ref{fig:one-qubit-shift}). Therefore, in order to obtain analytic polynomials of degree $\le n - 1$ we must choose $A_n$ such that $P_n$ and $Q_0$ become zero before applying $\Tilde{w}^\dag$, in other words
    \begin{align}
        \label{eq:single-qubit-reduction-condition}
        A_n^\dag
        \begin{bmatrix}
            P_n \\ Q_n
        \end{bmatrix}
        = 
        \begin{bmatrix}
            0 \\ a
        \end{bmatrix}
        = a \ket{1}, \ \ \ \ \ A_n^\dag
        \begin{bmatrix}
            P_0 \\ Q_0
        \end{bmatrix}
        = 
        \begin{bmatrix}
            b \\ 0
        \end{bmatrix}
        = b \ket{0}
    \end{align}
    for some $a, b \in \C$. Note that the resulting vectors are orthogonal to each other and, since unitaries preserve inner products, such $A_n$ exists if and only if $(P_n, Q_n)$ and $(P_0, Q_0)$ are orthogonal. Fortunately, this is implied by condition~(ii): $|P|^2 + |Q|^2 = 1$ holds as a polynomial equation, therefore every coefficient of degree $\neq 0$ must be equal to zero, and one can check that the $n$-th coefficient of this polynomial is exactly $P_0^* P_n + Q_0^* Q_n$, the inner product between the two coefficient vectors at the boundary. Under this orthogonality condition, a choice of $A_n$ that reduces the degree of $P, Q$ can be derived from Eq.~(\ref{eq:single-qubit-reduction-condition}):
    \begin{align*}
        A_n =
        \begin{bmatrix}
            P_0 / b & P_n / a \\
            Q_0 / b & Q_n / a
        \end{bmatrix}
    \end{align*}
    Of course, it could happen that $a$ (resp.\ $b$) is $0$. But in that case, since $A_n$ has full rank, it means that $P_n = Q_n = 0$ (resp.\ $P_0 = Q_0 = 0$), making one of the conditions in Eq.~(\ref{eq:single-qubit-reduction-condition}) vacuous. Therefore, we can simply choose $A_n$ to guarantee the other condition, and then choose the second column to be a unit vector orthogonal to the first. If both $a, b = 0$ then any $A_n$ will guarantee the degree reduction. Also in these cases, however, we can say that $(P_n, Q_n)$ and $(P_0, Q_0)$ are (trivially) orthogonal. 
\end{proof}

\noindent Therefore, the existence of a unitary matrix $A_n$ that allows us to carry out the induction step is guaranteed exactly by the orthogonality condition $P_0^* P_n + Q_0^* Q_n = 0$, which is in turn guaranteed by condition (ii) throughout the whole induction.
Equation~(\ref{eq:single-qubit-reduction-condition}) can be seen in a different way: one can also rewrite it as
\begin{align*}
    A_n^\dag
    \begin{bmatrix}
        P_{n-1} & P_n \\
        Q_{n-1} & Q_n
    \end{bmatrix}
    =
    \begin{bmatrix}
        \cdot & 0 \\
        \cdot & \cdot
    \end{bmatrix},\ \ \ \ \ 
    A_n^\dag
    \begin{bmatrix}
        P_0 & P_1 \\
        Q_0 & Q_1
    \end{bmatrix}
    =
    \begin{bmatrix}
        \cdot & \cdot \\
        0 & \cdot
    \end{bmatrix}
\end{align*}
i.e., a left-multiplication by $A_n^\dag$ transforms these two matrices into a lower- and an upper-triangular matrix, respectively. While this seems a complicated way to state the orthogonality condition, it will become more natural for the multiple-qubit case.

==> contents/graveyard.tex <==
% single-qubit case:
% k with 2k-length
% ceil(n/2) with n-length

% k(2^b - 1) with 2k-length
% ceil(n(2^b - 1)/2) with n-length
% so any polynomial vector of degree n can be obtained only within 2n steps

\noindent Here we provide a proof for Theorem~\ref{thm:multi-qubit-qsp-analytic}, also restated here for simplicity.
\begin{theorem*}
    Let $\{ P_x \}_{0 \le x < 2^b} \in \C[z]$. There exist $A_0, \ldots, A_n \in SU(2^b)$ such that:
    \begin{align*}
        A_n \Tilde{w}_b A_{n-1} \Tilde{w}_b \cdots \Tilde{w}_b A_0 \ket{0} = \sum_x P_x(z) \ket{x} =: \ket{\gamma}
    \end{align*}
    if and only if:
    \begin{enumerate}[(i)]
        \item $\deg P_x \le (2^b - 1)n$ for every $0 \le x < 2^b$;
        \item $\sum_x |P_x(z)|^2 = 1$ for every $z \in U(1)$;
        \item $\ket{\gamma}$ is strongly reducible.
    \end{enumerate}
\end{theorem*}
\noindent Before proving the result, we want to give some insights on the idea. Considering the two-qubit case, we will have four polynomials $P, Q, R, S$, and in the induction step we will undo the last operation
\begin{align*}
    (A_n \Tilde{w}_2)^\dag
    \begin{bmatrix}
        P \\ Q \\ R \\ S
    \end{bmatrix}
    =:
    \begin{bmatrix}
        P' \\ Q' \\ R' \\ S'
    \end{bmatrix}
\end{align*}
where we want $P', Q', R', S'$ to be of degree $\le 3(n - 1)$. Here it is insightful to consider the action of $\Tilde{w}_2^\dag$: analogously to the single-qubit case, where $\Tilde{w}$ shifts the coefficients of $Q$ by one place to the left (see Figure~\ref{fig:one-qubit-shift} and Eq.~\ref{eq:one-qubit-poly-shift}), one can see that the action of $\Tilde{w}_2^\dag$ on the vector $(P, Q, R, S)$ is to shift the coefficients of these four polynomials by $0, 1, 2$ and $3$ places, respectively (see Figure~\ref{fig:two-qubit-shift}).
\begin{figure}
    \centering
    \input{figures/two-qubit-shift}
    \caption{Action of $\Tilde{w}^\dag$ on the coefficients of the four polynomials. For example, since $\Tilde{w}^\dag$ maps $R(z) \rightarrow z^{-2} R(z)$, all the coefficients of $R$ are shifted by two positions to the left. The colored squares are the coefficients of $z^k$ for $k \not\in [0, 3(n-1)]$ after the application of $\Tilde{w}^\dag$. In order to reduce the degree of the polynomials, we need to choose $A_n^\dag$ such that the colored squares are mapped to $0$.}
    \label{fig:two-qubit-shift}
\end{figure}
Therefore, in order to reduce a polynomial vector by three degrees we need to transform the first four coefficient vectors (i.e., the matrix $\Gamma_0$) into an upper triangular matrix, and the last four (i.e., the matrix $\Gamma_*$) into a lower triangular matrix, before applying $\Tilde{w}_b^\dag$. Thus the task is to understand a necessary and sufficient condition for the existence of a unitary matrix $A_n$ such that
\begin{align*}
    A_n^\dag \Gamma_0 & \text{ is upper triangular,} \\
    A_n^\dag \Gamma_* & \text{ is lower triangular.}
\end{align*}
It turns out such $A_n$ exists if and only if $\Gamma_0^\dag \Gamma_*$ is lower triangular (proof in Appendix~\ref{apx:triangular-matrices}), giving us a characterization of weak reducibility for an arbitrary number of qubits.
\begin{proof}[Proof of Theorem~\ref{thm:multi-qubit-qsp-analytic}]
    For $n = 0$ we obtain $\ket{\gamma} = A_0 \ket{0}$, which trivially satisfies conditions (i)-(iii). For $n > 0$ then the first $n - 1$ steps give a polynomial state $\ket{\gamma'}$ satisfying the three conditions, by induction. Taking $\ket{\gamma} = A_n \Tilde{w}_b \ket{\gamma'}$, this new state satisfies condition (i) as $\Tilde{w}_b$ can only increase the degree by at most $2^b - 1$, condition (ii) is preserved by unitarity and a strongly reducible \TODO any or some reduction must be strongly reducible?? Is it possible to have non invertible triangular matrices in a strongly reducible polynomial?
\end{proof}

==> contents/low-algebra.tex <==
\section{Defining phase factors for multiple qubits}
\label{sec:low-algebra-attempts}

\noindent The construction of Theorem~\ref{thm:single-qubit-qsp-analytic} is quite general, but for ease of implementation, one usually restricts $A_n$ to be a rotation around a Pauli basis. The variant found the most in the literature usually refers to as the $W_x$-convention~\cite{martynGrandUnificationQuantum2021}, where the signal operator $\Tilde{w}$ is expressed in the $X$-basis (unlike our choice of using the $Z$-basis), while $A_k = e^{i\phi_k Z}$, and the only choice is the phase factor $\phi_k$ in this rotation matrix.
\begin{align}
    \label{eq:qsp-one-qubit-low-ansatz}
    e^{i \phi_n Z} H \Tilde{w} H e^{i \phi_{n-1} Z} H \Tilde{w} H \cdots H \Tilde{w} H e^{i \phi_0 Z}\ket{0} = 
    \begin{bmatrix}
        P(z) \\ Q(z)
    \end{bmatrix}
\end{align}
where $H$ is the Hadamard gate. This constraint on the $A_k$'s induces an additional condition on $P, Q$, namely that $P(z) = z^n P(z^{-1}), Q(z) = -z^n Q(z^{-1})$ (in the analytic picture), or $P(z) = P(z^{-1}), Q(z) = -Q(z^{-1})$ (in the Laurent picture), which is not restrictive in practice, as it can be circumvented with a linear combination of unitaries technique~\cite{berryHamiltonianSimulationNearly2015,childsHamiltonianSimulationUsing2012,childsQuantumAlgorithmSystems2017}.

Chao et al.~\cite{chaoFindingAnglesQuantum2020} highlighted that, in the Laurent picture, the construction of Eq.~(\ref{eq:qsp-one-qubit-low-ansatz}) generates all the unitary (parity) elements of a *-algebra, a subalgebra of the *-algebra whose unitary (parity) elements are generated by the product of Corollary~\ref{thm:single-qubit-qsp-laurent}.

In this section we show attempts to extend this simplified ansatz to the multiple-qubit setting, along with their subtleties, as different choices are possible by choosing different generalizations of the Pauli matrices.

\subsection{Naive construction using Hadamard transform}
A first idea would be to conjugate the $b$-qubit signal operator $\Tilde{w}_b = \diag(z^k)_{k \in [2^b]}$ with the $b$-fold Hadamard gate, while we take tensor products of $Z$-rotations as signal processing operators:
\begin{align*}
    \left(\bigotimes_{i=0}^b e^{i \phi_{i,n} Z} \right)
    H^{\otimes b} \Tilde{w}_b H^{\otimes b} \left(\bigotimes_{i=0}^b e^{i \phi_{i,n-1} Z} \right) \cdots \left(\bigotimes_{i=0}^b e^{i \phi_{i,1} Z} \right)
    H^{\otimes b} \Tilde{w}_b H^{\otimes b}
    \left(\bigotimes_{i=0}^b e^{i \phi_{i,0} Z} \right).
\end{align*}
In this case, we are essentially taking the $n$-fold Pauli matrices $X^{\otimes n}, Z^{\otimes n}$ as the multi-qubit extensions of $X, Z$, and at each step we must choose $b$ phase factors. This construction, however, gives trivial results: as every operator is written as tensor product, this multi-qubit QSP construction can be seen as $b$ parallel single-qubit QSP constructions, and the only polynomials that we can generate are of the form $P_1(z) P_2(z^2) \cdots P_n(z^{2^{b-1}})$
An example of polynomial vector not achievable in this way is the one from phase estimation (see Section~\ref{sec:phase-estimation}).

\subsection{Clock and shift construction using the quantum Fourier transform}
\noindent Instead of extending the Hadamard gate of Eq.~(\ref{eq:qsp-one-qubit-low-ansatz}) with a $b$-fold Hadamard gate, we replace it with $Q_{2^b}$, the $b$-qubit quantum Fourier transform.
\begin{align*}
    \left(\bigotimes_{i=0}^b e^{i \phi_{i,n} Z} \right) Q_{2^b} \Tilde{w}_b Q_{2^b}^\dag \left(\bigotimes_{i=0}^b e^{i \phi_{i,{n-1}} Z} \right)
    \cdots
    \left(\bigotimes_{i=0}^b e^{i \phi_{i,1} Z} \right) Q_{2^b} \Tilde{w}_b Q_{2^b}^\dag \left(\bigotimes_{i=0}^b e^{i \phi_{i,0} Z} \right)
\end{align*}
First of all, it is worth to remark that phase estimation is given by the most trivial sequence of this ansatz, where $n = 1$ and $\phi_{i,0} = \phi_{i,1} = 0$ for every $0 \le i < b$. The bases of the two types of operators are the ones of the clock and shift operators
\begin{align*}
    \Sigma_1 \ket{x} = \ket{(x+1) \bmod 2^b},\ \ \ \ 
    \Sigma_3 =
    \diag(e^{2\pi i k/2^b})_k
\end{align*}
which are alternative extensions of $X, Z$. An interesting property of this ansatz is that the $2^b$ polynomials $P_k(z)$ satisfy a symmetry constraint similar to the one for the single-qubit case: consider a signal operator of the form
\begin{align*}
    \Tilde{w}_b = \diag(z_k)_{0 \le k < 2^b}
\end{align*}
where $z_k$ are independent variables. This is the most generic construction: if we plug $z_k = z^k$ we obtain the analytic picture, while for $z_k = z^{k - 2^b + 1}$ the Laurent picture arises. In the single-qubit case we would have two polynomials $P(z_0, z_1), Q(z_0, z_1)$ such that
\begin{align*}
    P(z_1, z_0) & = P(z_0, z_1) \\
    Q(z_1, z_0) & = -Q(z_0, z_1)
\end{align*}
in other words, if we group the variables into a vector $\vec{z}$, then we can rewrite the swap of the two variables as $\vec{z} \rightarrow X\vec{z}$ (where in the Laurent picture it simply means $z \rightarrow z^{-1}$). In the general case, we replace $X$ with the shift operator $\Sigma_1$, thus obtaining
\begin{align*}
    P_i(\Sigma_1 \vec{z}) & = \omega_{2^b}^i P_i(\vec{z})
\end{align*}

==> figures/two-qubit-qsp-ansatz.tex <==
\begin{quantikz}
    \lstick[wires=2]{$\ket{0}$} & \gate[wires=2]{A_0} & \qw & \ctrl{2} & \gate[wires=2]{A_1} & \qw & \ctrl{2} & \ \ldots\ \qw  & \qw & \ctrl{2} & \gate[wires=2]{A_n} & \qw \\
    & & \ctrl{1} & \qw & & \ctrl{1} & \qw & \ \ldots\ \qw & \ctrl{1} & \qw & & \qw \\
    \lstick{$\ket{\psi}$} & \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \ \ldots\ \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \qwbundle[alternate]{} & \qwbundle[alternate]{}
\end{quantikz}

==> figures/two-qubit-qsp-exponential.tex <==
\begin{quantikz}
    \lstick[wires=2]{$\ket{0}$} & \gate[wires=2]{A_0} & \qw & \ctrl{2} & \gate[wires=2]{A_1} & \qw & \ctrl{2} & \ \ldots\ \qw  & \qw & \ctrl{2} & \gate[wires=2]{A_n} & \qw \\
    & & \ctrl{1} & \qw & & \ctrl{1} & \qw & \ \ldots\ \qw & \ctrl{1} & \qw & & \qw \\
    \lstick{$\ket{\psi}$} & \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \ \ldots\ \qwbundle[alternate]{} & \gate{U}\qwbundle[alternate]{} & \gate{U^2}\qwbundle[alternate]{} & \qwbundle[alternate]{} & \qwbundle[alternate]{}
\end{quantikz}

==> graveyard.tex <==
% single-qubit case:
% k with 2k-length
% ceil(n/2) with n-length

% k(2^b - 1) with 2k-length
% ceil(n(2^b - 1)/2) with n-length
% so any polynomial vector of degree n can be obtained only within 2n steps

\noindent Here we provide a proof for Theorem~\ref{thm:multi-qubit-qsp-analytic}, also restated here for simplicity.
\begin{theorem*}
    Let $\{ P_x \}_{0 \le x < 2^b} \in \C[z]$. There exist $A_0, \ldots, A_n \in SU(2^b)$ such that:
    \begin{align*}
        A_n \Tilde{w}_b A_{n-1} \Tilde{w}_b \cdots \Tilde{w}_b A_0 \ket{0} = \sum_x P_x(z) \ket{x} =: \ket{\gamma}
    \end{align*}
    if and only if:
    \begin{enumerate}[(i)]
        \item $\deg P_x \le (2^b - 1)n$ for every $0 \le x < 2^b$;
        \item $\sum_x |P_x(z)|^2 = 1$ for every $z \in U(1)$;
        \item $\ket{\gamma}$ is strongly reducible.
    \end{enumerate}
\end{theorem*}
\noindent Before proving the result, we want to give some insights on the idea. Considering the two-qubit case, we will have four polynomials $P, Q, R, S$, and in the induction step we will undo the last operation
\begin{align*}
    (A_n \Tilde{w}_2)^\dag
    \begin{bmatrix}
        P \\ Q \\ R \\ S
    \end{bmatrix}
    =:
    \begin{bmatrix}
        P' \\ Q' \\ R' \\ S'
    \end{bmatrix}
\end{align*}
where we want $P', Q', R', S'$ to be of degree $\le 3(n - 1)$. Here it is insightful to consider the action of $\Tilde{w}_2^\dag$: analogously to the single-qubit case, where $\Tilde{w}$ shifts the coefficients of $Q$ by one place to the left (see Figure~\ref{fig:one-qubit-shift} and Eq.~\ref{eq:one-qubit-poly-shift}), one can see that the action of $\Tilde{w}_2^\dag$ on the vector $(P, Q, R, S)$ is to shift the coefficients of these four polynomials by $0, 1, 2$ and $3$ places, respectively (see Figure~\ref{fig:two-qubit-shift}).
\begin{figure}
    \centering
    \input{figures/two-qubit-shift}
    \caption{Action of $\Tilde{w}^\dag$ on the coefficients of the four polynomials. For example, since $\Tilde{w}^\dag$ maps $R(z) \rightarrow z^{-2} R(z)$, all the coefficients of $R$ are shifted by two positions to the left. The colored squares are the coefficients of $z^k$ for $k \not\in [0, 3(n-1)]$ after the application of $\Tilde{w}^\dag$. In order to reduce the degree of the polynomials, we need to choose $A_n^\dag$ such that the colored squares are mapped to $0$.}
    \label{fig:two-qubit-shift}
\end{figure}
Therefore, in order to reduce a polynomial vector by three degrees we need to transform the first four coefficient vectors (i.e., the matrix $\Gamma_0$) into an upper triangular matrix, and the last four (i.e., the matrix $\Gamma_*$) into a lower triangular matrix, before applying $\Tilde{w}_b^\dag$. Thus the task is to understand a necessary and sufficient condition for the existence of a unitary matrix $A_n$ such that
\begin{align*}
    A_n^\dag \Gamma_0 & \text{ is upper triangular,} \\
    A_n^\dag \Gamma_* & \text{ is lower triangular.}
\end{align*}
It turns out such $A_n$ exists if and only if $\Gamma_0^\dag \Gamma_*$ is lower triangular (proof in Appendix~\ref{apx:triangular-matrices}), giving us a characterization of weak reducibility for an arbitrary number of qubits.
\begin{proof}[Proof of Theorem~\ref{thm:multi-qubit-qsp-analytic}]
    For $n = 0$ we obtain $\ket{\gamma} = A_0 \ket{0}$, which trivially satisfies conditions (i)-(iii). For $n > 0$ then the first $n - 1$ steps give a polynomial state $\ket{\gamma'}$ satisfying the three conditions, by induction. Taking $\ket{\gamma} = A_n \Tilde{w}_b \ket{\gamma'}$, this new state satisfies condition (i) as $\Tilde{w}_b$ can only increase the degree by at most $2^b - 1$, condition (ii) is preserved by unitarity and a strongly reducible \TODO any or some reduction must be strongly reducible?? Is it possible to have non invertible triangular matrices in a strongly reducible polynomial?
\end{proof}
